Mitigating Multilingual Hallucination in Large Vision-Language Models

While Large Vision-Language Models (LVLMs) have exhibited remarkable capabilities across a wide range of tasks, they suffer from hallucination problems, where models generate plausible yet incorrect answers given the input image-query pair. This hallucination phenomenon is even more severe when querying the image in non-English languages, while existing methods for mitigating hallucinations in LVLMs only consider the English scenarios. In this paper, we make the first attempt to mitigate this important multilingual hallucination in LVLMs. With thorough experiment analysis, we found that multilingual hallucination in LVLMs is a systemic problem that could arise from deficiencies in multilingual capabilities or inadequate multimodal abilities. To this end, we propose a two-stage Multilingual Hallucination Removal (MHR) framework for LVLMs, aiming to improve resistance to hallucination for both high-resource and low-resource languages. Instead of relying on the intricate manual annotations of multilingual resources, we fully leverage the inherent capabilities of the LVLM and propose a novel cross-lingual alignment method, which generates multiple responses for each image-query input and then identifies the hallucination-aware pairs for each language. These data pairs are finally used for direct preference optimization to prompt the LVLMs to favor non-hallucinating responses. Experimental results show that our MHR achieves a substantial reduction in hallucination generation for LVLMs. Notably, on our extended multilingual POPE benchmark, our framework delivers an average increase of 19.0% in accuracy across 13 different languages. Our code and model weights are available at https://github.com/ssmisya/MHR

==> tables/full_results_on_ablation_study_ratio.tex <==

\newcommand{\smallcircle}{\tikz\draw (0,0) circle (.5ex);}
\onecolumn
\begin{longtable}{c ccc ||ccc|c || ccc|c || ccc|c}
\caption{Full result for ablation study on different datasets, namely explicitly hallucination-aware dataset $D_e^h$ (emp.), implicitly hallucination-aware dataset $D_i^h$(imp.) and translated multilingual dataset $D_t^h$(trans.). Our evaluation is conducted on the `popular' dataset subset. Average scores are indicated in a \colorbox{gray!20}{gray} shade while the top accuracy results are highlighted in bold.} \\
\hline
&\multicolumn{3}{c||}{Dataset.} & \multicolumn{4}{c||}{MS COCO} & \multicolumn{4}{c||}{AOKVQA} & \multicolumn{4}{c}{GQA}\\
\textbf{lang.}& $D_e^h$&$D_i^h$&$D_t^h$ &Precision & Recall & F1 & Acc. & Precision & Recall & F1 & Acc. & Precision & Recall & F1 & Acc. \\
\hline
\hline
\endfirsthead  % 第一页表头的末尾

\multicolumn{14}{c}{\textit{\tablename\ \thetable{} -- \textit{Continued from previous page}}} \\ 
\hline
&\multicolumn{3}{c||}{Dataset.} & \multicolumn{4}{c||}{MS COCO} & \multicolumn{4}{c||}{AOKVQA} & \multicolumn{4}{c}{GQA}\\
\textbf{lang.}& $D_e^h$&$D_i^h$&$D_t^h$ &Precision & Recall & F1 & Acc. & Precision & Recall & F1 & Acc. & Precision & Recall & F1 & Acc.\\
\hline 
\endhead  % 接下来页表头的末尾

\hline 
\multicolumn{14}{r}{\textit{shown in next page}} \\ 
\endfoot  % 每页表尾


\endlastfoot  % 最后一页表尾



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%% AUTO GENERATE AREA %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\multicolumn{16}{c}{\textbf{High Resource Languages (HRL)}} \\   \hline 
 \multirow{9}{*}{\centering \textbf{en}} 
 & \checkmark & \smallcircle  &\smallcircle & 96.6 & 73.9 & 83.8 & 85.7 & 90.8 & 81.1 & 85.7 & 86.4 & 86.6 & 79.5 & 82.9 & 83.6 \\ 
& \smallcircle & \checkmark  &\smallcircle & 96.9 & 74.0 & 83.9 & 85.8 & 91.4 & 81.2 & 86.0 & 86.8 & 87.6 & 78.8 & 82.9 & \textbf{83.8} \\ 
& \smallcircle & \smallcircle  &\checkmark & 96.6 & 74.2 & 83.9 & 85.8 & 89.4 & 81.2 & 85.1 & 85.8 & 83.7 & 79.7 & 81.7 & 82.1 \\ 
& \checkmark & \checkmark  &\smallcircle & 96.9 & 74.4 & 84.2 & 86.0 & 91.1 & 80.7 & 85.6 & 86.4 & 87.1 & 79.0 & 82.9 & 83.7 \\ 
& \smallcircle & \checkmark  &\checkmark & 97.4 & 70.5 & 81.8 & 84.3 & 91.5 & 77.8 & 84.1 & 85.3 & 87.6 & 76.7 & 81.8 & 82.9 \\ 
& \checkmark & \smallcircle  &\checkmark & 97.4 & 72.0 & 82.8 & 85.0 & 91.2 & 79.1 & 84.7 & 85.7 & 87.0 & 77.8 & 82.1 & 83.1 \\ 
& \checkmark & \checkmark  &\checkmark & 97.3 & 70.7 & 81.9 & 84.4 & 91.8 & 77.3 & 83.9 & 85.2 & 87.6 & 76.1 & 81.4 & 82.6 \\ 
& \multicolumn{3}{c||}{--- SFT LLaVA ---} & 95.8 & 76.4 & 85.0 & \textbf{86.5} & 89.6 & 83.5 & 86.4 & \textbf{86.9} & 84.8 & 80.8 & 82.8 & 83.2 \\ 
& \multicolumn{3}{c||}{--- Base LLaVA ---} & 94.6 & 78.1 & 85.6 & 86.0 & 87.9 & 87.0 & 87.4 & 86.8 & 83.0 & 84.0 & 83.5 & 82.8 \\ 
\hline 
 \multirow{9}{*}{\centering \textbf{ru}} 
 & \checkmark & \smallcircle  &\smallcircle & 65.6 & 96.6 & 78.1 & 72.9 & 58.5 & 99.3 & 73.6 & 64.4 & 56.0 & 99.1 & 71.6 & 60.6 \\ 
& \smallcircle & \checkmark  &\smallcircle & 72.7 & 95.1 & 82.4 & 79.5 & 61.5 & 98.3 & 75.6 & 68.2 & 56.9 & 98.8 & 72.2 & 61.9 \\ 
& \smallcircle & \smallcircle  &\checkmark & 66.3 & 95.8 & 78.4 & 73.6 & 60.0 & 99.3 & 74.8 & 66.5 & 56.4 & 98.7 & 71.8 & 61.3 \\ 
& \checkmark & \checkmark  &\smallcircle & 71.8 & 95.9 & 82.1 & 78.9 & 60.2 & 98.9 & 74.8 & 66.7 & 56.5 & 99.0 & 72.0 & 61.4 \\ 
& \smallcircle & \checkmark  &\checkmark & 81.1 & 90.6 & 85.6 & 84.3 & 65.3 & 95.7 & 77.6 & \textbf{72.3} & 58.7 & 96.8 & 73.0 & 64.2 \\ 
& \checkmark & \smallcircle  &\checkmark & 75.4 & 94.0 & 83.7 & 81.7 & 62.8 & 98.5 & 76.7 & 70.0 & 58.1 & 98.7 & 73.2 & 63.8 \\ 
& \checkmark & \checkmark  &\checkmark & 80.7 & 91.5 & 85.8 & \textbf{84.5} & 64.8 & 96.6 & 77.6 & 72.0 & 58.7 & 97.3 & 73.2 & \textbf{64.3} \\ 
& \multicolumn{3}{c||}{--- SFT LLaVA ---} & 59.7 & 97.7 & 74.1 & 65.8 & 55.9 & 99.7 & 71.7 & 60.6 & 54.2 & 99.7 & 70.3 & 57.8 \\ 
& \multicolumn{3}{c||}{--- Base LLaVA ---} & 53.6 & 98.4 & 69.4 & 55.9 & 52.1 & 99.9 & 68.5 & 53.9 & 52.6 & 99.7 & 68.9 & 54.8 \\ 
\hline 
 \multirow{9}{*}{\centering \textbf{de}} 
 & \checkmark & \smallcircle  &\smallcircle & 95.5 & 71.5 & 81.8 & 84.1 & 88.9 & 72.2 & 79.7 & 81.6 & 80.8 & 71.8 & 76.0 & 77.4 \\ 
& \smallcircle & \checkmark  &\smallcircle & 95.1 & 74.7 & 83.6 & 85.4 & 87.7 & 76.3 & 81.6 & 82.8 & 80.1 & 74.1 & 77.0 & 77.9 \\ 
& \smallcircle & \smallcircle  &\checkmark & 94.0 & 78.5 & 85.6 & 86.8 & 85.5 & 79.3 & 82.3 & 82.9 & 77.8 & 78.9 & 78.4 & 78.2 \\ 
& \checkmark & \checkmark  &\smallcircle & 95.4 & 75.3 & 84.1 & 85.8 & 87.7 & 77.0 & 82.0 & 83.1 & 80.4 & 75.7 & 78.0 & \textbf{78.6} \\ 
& \smallcircle & \checkmark  &\checkmark & 96.0 & 72.0 & 82.3 & 84.5 & 89.6 & 73.4 & 80.7 & 82.4 & 81.6 & 72.0 & 76.5 & 77.9 \\ 
& \checkmark & \smallcircle  &\checkmark & 95.6 & 73.2 & 82.9 & 84.9 & 88.2 & 73.6 & 80.3 & 81.9 & 80.3 & 73.5 & 76.7 & 77.7 \\ 
& \checkmark & \checkmark  &\checkmark & 96.6 & 70.5 & 81.5 & 84.0 & 88.8 & 70.5 & 78.6 & 80.8 & 81.9 & 71.1 & 76.1 & 77.7 \\ 
& \multicolumn{3}{c||}{--- SFT LLaVA ---} & 93.6 & 80.9 & 86.8 & \textbf{87.7} & 86.1 & 80.7 & 83.3 & \textbf{83.8} & 78.1 & 79.0 & 78.5 & 78.4 \\ 
& \multicolumn{3}{c||}{--- Base LLaVA ---} & 95.2 & 75.0 & 83.9 & 83.3 & 88.6 & 73.3 & 80.2 & 80.4 & 80.4 & 72.8 & 76.4 & 75.8 \\ 
\hline 
 \multirow{9}{*}{\centering \textbf{zh}} 
 & \checkmark & \smallcircle  &\smallcircle & 71.8 & 95.9 & 82.1 & 79.1 & 62.0 & 98.9 & 76.2 & 69.1 & 59.5 & 99.2 & 74.4 & 65.8 \\ 
& \smallcircle & \checkmark  &\smallcircle & 77.6 & 97.0 & 86.2 & 66.5 & 64.5 & 99.0 & 78.1 & 61.6 & 60.4 & 99.1 & 75.1 & 61.2 \\ 
& \smallcircle & \smallcircle  &\checkmark & 83.6 & 93.1 & 88.1 & \textbf{87.4} & 71.0 & 96.6 & 81.9 & \textbf{78.6} & 66.3 & 95.9 & 78.4 & \textbf{73.6} \\ 
& \checkmark & \checkmark  &\smallcircle & 75.9 & 94.8 & 84.3 & 82.3 & 64.0 & 98.3 & 77.5 & 71.5 & 60.8 & 98.5 & 75.2 & 67.5 \\ 
& \smallcircle & \checkmark  &\checkmark & 84.6 & 89.5 & 87.0 & 86.4 & 69.9 & 95.4 & 80.7 & 77.1 & 64.9 & 95.7 & 77.3 & 71.9 \\ 
& \checkmark & \smallcircle  &\checkmark & 82.5 & 93.2 & 87.5 & 86.7 & 69.5 & 97.0 & 81.0 & 77.2 & 64.5 & 97.3 & 77.6 & 71.9 \\ 
& \checkmark & \checkmark  &\checkmark & 83.4 & 91.3 & 87.1 & 86.5 & 67.8 & 96.2 & 79.5 & 75.2 & 63.0 & 97.0 & 76.4 & 70.0 \\ 
& \multicolumn{3}{c||}{--- SFT LLaVA ---} & 66.7 & 97.6 & 79.2 & 74.4 & 58.8 & 99.5 & 73.9 & 64.8 & 57.4 & 99.6 & 72.8 & 62.8 \\ 
& \multicolumn{3}{c||}{--- Base LLaVA ---} & 50.0 & 100.0 & 66.6 & 47.8 & 49.9 & 100.0 & 66.6 & 48.1 & 49.5 & 100.0 & 66.2 & 47.6 \\ 
\hline 
 \multirow{9}{*}{\centering \textbf{ja}} 
 & \checkmark & \smallcircle  &\smallcircle & 80.5 & 90.9 & 85.4 & 84.5 & 63.4 & 95.3 & 76.1 & 70.1 & 58.7 & 96.3 & 72.9 & 64.2 \\ 
& \smallcircle & \checkmark  &\smallcircle & 83.6 & 88.8 & 86.1 & 85.6 & 64.3 & 94.3 & 76.4 & 70.9 & 58.8 & 95.2 & 72.7 & 64.2 \\ 
& \smallcircle & \smallcircle  &\checkmark & 79.9 & 92.9 & 85.9 & 84.7 & 63.0 & 96.5 & 76.2 & 69.9 & 57.5 & 97.5 & 72.4 & 62.7 \\ 
& \checkmark & \checkmark  &\smallcircle & 79.9 & 91.4 & 85.3 & 84.2 & 63.3 & 96.3 & 76.4 & 70.2 & 58.4 & 97.0 & 72.9 & 63.9 \\ 
& \smallcircle & \checkmark  &\checkmark & 84.4 & 88.5 & 86.4 & 86.0 & 63.9 & 92.1 & 75.4 & 70.0 & 58.1 & 94.4 & 71.9 & 63.2 \\ 
& \checkmark & \smallcircle  &\checkmark & 88.4 & 84.0 & 86.2 & \textbf{86.5} & 68.7 & 89.2 & 77.6 & \textbf{74.3} & 63.9 & 89.7 & 74.6 & \textbf{69.5} \\ 
& \checkmark & \checkmark  &\checkmark & 86.2 & 86.5 & 86.3 & 86.3 & 65.6 & 91.9 & 76.6 & 71.9 & 60.5 & 92.3 & 73.1 & 66.1 \\ 
& \multicolumn{3}{c||}{--- SFT LLaVA ---} & 74.1 & 94.5 & 83.1 & 80.7 & 59.8 & 98.2 & 74.3 & 66.1 & 55.6 & 98.3 & 71.0 & 59.9 \\ 
& \multicolumn{3}{c||}{--- Base LLaVA ---} & 51.2 & 100.0 & 67.7 & 49.1 & 49.9 & 100.0 & 66.6 & 48.3 & 49.6 & 100.0 & 66.3 & 47.5 \\ 
\hline 
 \multirow{3}{*}{\centering \textbf{fr}} 
 & \checkmark & \smallcircle  &\smallcircle & 73.1 & 95.9 & 83.0 & 80.3 & 64.4 & 98.7 & 77.9 & 72.0 & 59.8 & 99.1 & 74.6 & 66.2 \\ 
& \smallcircle & \checkmark  &\smallcircle & 79.4 & 93.7 & 86.0 & 84.7 & 67.8 & 97.4 & 79.9 & 75.6 & 62.1 & 98.5 & 76.2 & 69.2 \\ 
& \smallcircle & \smallcircle  &\checkmark & 78.9 & 94.2 & 85.8 & 84.5 & 68.8 & 97.2 & 80.6 & 76.6 & 63.3 & 98.2 & 77.0 & 70.6 \\ 
 \multirow{6}{*}{\centering \textbf{fr}} & \checkmark & \checkmark  &\smallcircle & 79.2 & 94.1 & 86.0 & 84.7 & 67.6 & 97.7 & 79.9 & 75.4 & 61.8 & 98.7 & 76.0 & 68.9 \\ 
& \smallcircle & \checkmark  &\checkmark & 85.6 & 89.7 & 87.6 & 87.3 & 69.7 & 94.9 & 80.4 & 76.8 & 63.3 & 96.2 & 76.3 & 70.2 \\ 
& \checkmark & \smallcircle  &\checkmark & 81.6 & 93.4 & 87.1 & 86.2 & 68.7 & 96.9 & 80.4 & 76.4 & 62.5 & 98.1 & 76.3 & 69.6 \\ 
& \checkmark & \checkmark  &\checkmark & 84.7 & 91.4 & 87.9 & \textbf{87.5} & 69.9 & 95.7 & 80.8 & \textbf{77.3} & 63.6 & 97.2 & 76.9 & \textbf{70.7} \\ 
& \multicolumn{3}{c||}{--- SFT LLaVA ---} & 70.1 & 96.9 & 81.4 & 77.8 & 62.8 & 99.1 & 76.9 & 70.2 & 58.8 & 99.6 & 74.0 & 64.9 \\ 
& \multicolumn{3}{c||}{--- Base LLaVA ---} & 63.7 & 97.9 & 77.2 & 70.9 & 62.4 & 99.4 & 76.7 & 69.6 & 58.5 & 99.5 & 73.7 & 64.3 \\ 
\hline 
 \multirow{9}{*}{\centering \textbf{es}} 
 & \checkmark & \smallcircle  &\smallcircle & 91.1 & 82.3 & 86.5 & 87.1 & 80.8 & 88.1 & 84.3 & 83.6 & 75.0 & 87.8 & 80.9 & 79.3 \\ 
& \smallcircle & \checkmark  &\smallcircle & 91.7 & 82.9 & 87.1 & 87.0 & 80.6 & 89.4 & 84.8 & 83.9 & 72.9 & 89.5 & 80.3 & 77.9 \\ 
& \smallcircle & \smallcircle  &\checkmark & 91.0 & 83.4 & 87.1 & 87.6 & 80.1 & 88.5 & 84.1 & 83.3 & 73.9 & 88.0 & 80.3 & 78.4 \\ 
& \checkmark & \checkmark  &\smallcircle & 92.3 & 81.3 & 86.5 & 87.0 & 82.3 & 87.1 & 84.7 & \textbf{84.2} & 75.8 & 86.8 & 81.0 & \textbf{79.5} \\ 
& \smallcircle & \checkmark  &\checkmark & 93.8 & 78.0 & 85.2 & 85.9 & 80.9 & 85.6 & 83.2 & 82.7 & 73.0 & 85.2 & 78.6 & 76.7 \\ 
& \checkmark & \smallcircle  &\checkmark & 92.5 & 80.2 & 85.9 & 86.8 & 81.5 & 86.0 & 83.7 & 83.2 & 75.4 & 85.5 & 80.2 & 78.8 \\ 
& \checkmark & \checkmark  &\checkmark & 94.9 & 76.5 & 84.7 & 85.6 & 82.7 & 83.9 & 83.3 & 83.1 & 75.4 & 84.4 & 79.6 & 78.2 \\ 
& \multicolumn{3}{c||}{--- SFT LLaVA ---} & 87.9 & 87.5 & 87.7 & \textbf{87.8} & 77.5 & 92.5 & 84.4 & 82.8 & 71.9 & 92.6 & 81.0 & 78.2 \\ 
& \multicolumn{3}{c||}{--- Base LLaVA ---} & 97.7 & 47.7 & 64.1 & 73.2 & 95.9 & 48.3 & 64.2 & 73.0 & 95.8 & 47.3 & 63.3 & 72.6 \\ 
\hline 
 \multirow{9}{*}{\centering \textbf{pt}} 
 & \checkmark & \smallcircle  &\smallcircle & 72.8 & 94.9 & 82.4 & 79.8 & 64.3 & 98.3 & 77.7 & 71.9 & 60.2 & 98.5 & 74.7 & 66.6 \\ 
& \smallcircle & \checkmark  &\smallcircle & 77.6 & 92.1 & 84.2 & 82.8 & 67.9 & 96.5 & 79.7 & 75.4 & 61.8 & 97.5 & 75.6 & 68.6 \\ 
& \smallcircle & \smallcircle  &\checkmark & 75.2 & 94.5 & 83.7 & 81.6 & 68.0 & 97.3 & 80.0 & \textbf{75.7} & 63.3 & 98.1 & 77.0 & \textbf{70.7} \\ 
& \checkmark & \checkmark  &\smallcircle & 77.1 & 93.3 & 84.4 & 82.8 & 67.0 & 97.2 & 79.3 & 74.6 & 61.2 & 97.5 & 75.2 & 67.9 \\ 
& \smallcircle & \checkmark  &\checkmark & 82.0 & 89.5 & 85.6 & \textbf{84.9} & 68.2 & 94.7 & 79.3 & 75.3 & 61.4 & 95.1 & 74.6 & 67.6 \\ 
& \checkmark & \smallcircle  &\checkmark & 78.1 & 93.2 & 85.0 & 83.6 & 67.0 & 96.7 & 79.2 & 74.6 & 61.6 & 97.4 & 75.5 & 68.4 \\ 
& \checkmark & \checkmark  &\checkmark & 80.8 & 91.0 & 85.6 & 84.7 & 67.5 & 95.3 & 79.0 & 74.7 & 61.2 & 96.2 & 74.8 & 67.6 \\ 
& \multicolumn{3}{c||}{--- SFT LLaVA ---} & 67.6 & 96.8 & 79.6 & 75.2 & 61.0 & 99.1 & 75.5 & 67.9 & 57.9 & 99.6 & 73.2 & 63.6 \\ 
& \multicolumn{3}{c||}{--- Base LLaVA ---} & 64.4 & 97.8 & 77.7 & 70.8 & 60.5 & 99.5 & 75.2 & 66.6 & 57.5 & 99.7 & 73.0 & 62.6 \\ 
\hline 
 \multirow{9}{*}{\centering \textbf{Avg.}} 
 & \rowcolor{gray!20} \checkmark & \smallcircle  &\smallcircle & 80.9 & 87.8 & 82.9 & 81.7 & 71.6 & 91.5 & 78.9 & 74.9 & 67.1 & 91.4 & 76.0 & 70.5 \\ 
& \rowcolor{gray!20} \smallcircle & \checkmark  &\smallcircle & 84.3 & 87.3 & 84.9 & 82.2 & 73.2 & 91.5 & 80.3 & 75.7 & 67.6 & 91.4 & 76.5 & 70.6 \\ 
& \rowcolor{gray!20} \smallcircle & \smallcircle  &\checkmark & 83.2 & 88.3 & 84.8 & 84.0 & 73.2 & 92.0 & 80.6 & 77.4 & 67.8 & 91.9 & 77.1 & 72.2 \\ 
& \rowcolor{gray!20} \checkmark & \checkmark  &\smallcircle & 83.6 & 87.6 & 84.6 & 84.0 & 72.9 & 91.7 & 80.0 & 76.5 & 67.8 & 91.5 & 76.6 & 71.4 \\ 
& \rowcolor{gray!20} \smallcircle & \checkmark  &\checkmark & 88.1 & 83.5 & 85.2 & \textbf{85.5} & 74.9 & 88.7 & 80.2 & 77.7 & 68.6 & 89.0 & 76.3 & 71.8 \\ 
& \rowcolor{gray!20} \checkmark & \smallcircle  &\checkmark & 86.4 & 85.4 & 85.1 & 85.2 & 74.7 & 89.6 & 80.4 & \textbf{77.9} & 69.2 & 89.7 & 77.0 & \textbf{72.8} \\ 
& \rowcolor{gray!20} \checkmark & \checkmark  &\checkmark & 88.1 & 83.7 & 85.1 & 85.4 & 74.8 & 88.4 & 79.9 & 77.5 & 69.0 & 89.0 & 76.4 & 72.2 \\ 
&  \multicolumn{3}{c||}{\cellcolor{gray!20}--- SFT LLaVA ---} & \rowcolor{gray!20} 77.0 & 91.0 & 82.1 & 79.5 & 68.9 & 94.1 & 78.3 & 72.9 & 64.8 & 93.6 & 75.4 & 68.6 \\ 
& \multicolumn{3}{c||}{\cellcolor{gray!20}--- Base LLaVA ---} & \rowcolor{gray!20} 71.3 & 86.9 & 74.0 & 67.1 & 68.4 & 88.4 & 73.2 & 65.8 & 65.9 & 87.9 & 71.4 & 63.5 \\ 
\hline 
\multicolumn{16}{c}{\textbf{Low Resource Languages (LRL)}} \\  \hline 
 \multirow{9}{*}{\centering \textbf{uk}} 
 & \checkmark & \smallcircle  &\smallcircle & 49.5 & 99.7 & 66.1 & 48.6 & 49.4 & 99.8 & 66.1 & 48.6 & 49.5 & 99.9 & 66.2 & 48.5 \\ 
& \smallcircle & \checkmark  &\smallcircle & 39.5 & 84.6 & 53.8 & 16.4 & 39.0 & 87.1 & 53.8 & 17.2 & 40.6 & 84.9 & 54.9 & 18.4 \\ 
& \smallcircle & \smallcircle  &\checkmark & 49.8 & 98.5 & 66.1 & 48.9 & 49.4 & 98.8 & 65.9 & \textbf{48.7} & 49.6 & 98.7 & 66.0 & \textbf{48.5} \\ 
& \checkmark & \checkmark  &\smallcircle & 49.1 & 99.5 & 65.8 & 47.5 & 48.8 & 99.7 & 65.5 & 47.5 & 49.0 & 99.4 & 65.7 & 47.5 \\ 
& \smallcircle & \checkmark  &\checkmark & 45.5 & 95.8 & 61.7 & 25.6 & 43.7 & 98.0 & 60.5 & 22.0 & 44.4 & 98.8 & 61.2 & 23.4 \\ 
& \checkmark & \smallcircle  &\checkmark & 49.7 & 99.5 & 66.3 & 48.8 & 49.4 & 99.4 & 66.0 & 48.2 & 49.5 & 99.7 & 66.1 & 47.9 \\ 
& \checkmark & \checkmark  &\checkmark & 50.4 & 98.7 & 66.8 & \textbf{49.3} & 49.5 & 99.5 & 66.1 & 48.4 & 49.6 & 99.4 & 66.2 & 48.1 \\ 
& \multicolumn{3}{c||}{--- SFT LLaVA ---} & 49.5 & 99.5 & 66.1 & 48.5 & 49.3 & 99.6 & 66.0 & 48.6 & 49.4 & 99.5 & 66.0 & 48.4 \\ 
& \multicolumn{3}{c||}{--- Base LLaVA ---} & 41.6 & 100.0 & 58.8 & 16.8 & 49.7 & 100.0 & 66.4 & 18.2 & 52.3 & 100.0 & 68.7 & 18.3 \\ 
\hline 
 \multirow{9}{*}{\centering \textbf{bg}} 
 & \checkmark & \smallcircle  &\smallcircle & 54.4 & 98.2 & 70.0 & 57.9 & 53.6 & 99.8 & 69.7 & 56.6 & 53.1 & 99.3 & 69.2 & 55.8 \\ 
& \smallcircle & \checkmark  &\smallcircle & 55.7 & 97.6 & 70.9 & 58.4 & 55.2 & 99.5 & 71.1 & 57.2 & 54.8 & 99.4 & 70.6 & 55.6 \\ 
& \smallcircle & \smallcircle  &\checkmark & 53.9 & 97.9 & 69.5 & 57.1 & 54.1 & 99.7 & 70.1 & 57.6 & 53.8 & 99.5 & 69.9 & 57.1 \\ 
& \checkmark & \checkmark  &\smallcircle & 56.4 & 97.3 & 71.4 & 60.9 & 55.6 & 99.5 & 71.3 & 59.6 & 54.2 & 99.3 & 70.1 & 57.1 \\ 
& \smallcircle & \checkmark  &\checkmark & 63.8 & 93.2 & 75.7 & 66.8 & 66.1 & 95.4 & 78.1 & \textbf{66.4} & 62.6 & 97.6 & 76.3 & 60.0 \\ 
& \checkmark & \smallcircle  &\checkmark & 56.8 & 96.4 & 71.5 & 61.5 & 56.9 & 99.3 & 72.3 & 62.0 & 55.1 & 99.1 & 70.8 & 59.2 \\ 
& \checkmark & \checkmark  &\checkmark & 63.2 & 92.8 & 75.2 & \textbf{68.5} & 61.9 & 95.5 & 75.1 & 66.2 & 58.9 & 97.4 & 73.4 & \textbf{61.4} \\ 
& \multicolumn{3}{c||}{--- SFT LLaVA ---} & 51.4 & 99.5 & 67.8 & 52.6 & 51.4 & 100.0 & 67.9 & 52.7 & 51.3 & 99.9 & 67.8 & 52.5 \\ 
& \multicolumn{3}{c||}{--- Base LLaVA ---} & 49.8 & 100.0 & 66.5 & 48.7 & 49.3 & 100.0 & 66.0 & 48.5 & 49.3 & 100.0 & 66.0 & 48.5 \\ 
\hline 
 \multirow{1}{*}{\centering \textbf{tr}} 
 & \checkmark & \smallcircle  &\smallcircle & 88.3 & 57.1 & 69.4 & 74.8 & 82.6 & 61.4 & 70.4 & 74.1 & 77.0 & 57.4 & 65.8 & 70.1 \\ 
 \multirow{8}{*}{\centering \textbf{tr}} & \smallcircle & \checkmark  &\smallcircle & 96.7 & 23.9 & 38.3 & 61.5 & 92.0 & 27.0 & 41.7 & 62.2 & 90.3 & 25.4 & 39.6 & 61.2 \\ 
& \smallcircle & \smallcircle  &\checkmark & 81.4 & 65.7 & 72.7 & 75.0 & 77.5 & 69.0 & 73.0 & \textbf{74.2} & 72.7 & 68.1 & 70.4 & \textbf{71.0} \\ 
& \checkmark & \checkmark  &\smallcircle & 92.9 & 39.7 & 55.6 & 68.3 & 87.9 & 41.8 & 56.7 & 67.9 & 84.6 & 38.6 & 53.0 & 65.6 \\ 
& \smallcircle & \checkmark  &\checkmark & 89.3 & 57.4 & 69.9 & 74.9 & 80.7 & 57.7 & 67.3 & 71.3 & 76.0 & 54.2 & 63.2 & 67.7 \\ 
& \checkmark & \smallcircle  &\checkmark & 87.6 & 59.1 & 70.6 & \textbf{75.2} & 80.7 & 62.5 & 70.4 & 73.7 & 76.3 & 57.5 & 65.6 & 69.7 \\ 
& \checkmark & \checkmark  &\checkmark & 89.3 & 50.1 & 64.2 & 71.6 & 82.5 & 53.9 & 65.2 & 70.3 & 79.3 & 50.4 & 61.6 & 67.7 \\ 
& \multicolumn{3}{c||}{--- SFT LLaVA ---} & 90.5 & 46.5 & 61.4 & 70.8 & 85.0 & 49.5 & 62.6 & 70.3 & 82.3 & 44.3 & 57.6 & 67.3 \\ 
& \multicolumn{3}{c||}{--- Base LLaVA ---} & 0.0 & 0.0 & 0.0 & 49.7 & 0.0 & 0.0 & 0.0 & 49.9 & 0.0 & 0.0 & 0.0 & 49.7 \\ 
\hline 
 \multirow{9}{*}{\centering \textbf{ar}} 
 & \checkmark & \smallcircle  &\smallcircle & 85.0 & 91.3 & 88.1 & \textbf{87.6} & 71.3 & 93.3 & 80.8 & 77.9 & 64.1 & 95.4 & 76.7 & 71.0 \\ 
& \smallcircle & \checkmark  &\smallcircle & 81.7 & 92.1 & 86.6 & 85.7 & 71.0 & 94.3 & 81.0 & 77.9 & 63.4 & 96.3 & 76.4 & 70.3 \\ 
& \smallcircle & \smallcircle  &\checkmark & 86.2 & 87.7 & 87.0 & 86.8 & 72.7 & 89.7 & 80.3 & 78.0 & 65.4 & 90.8 & 76.0 & 71.4 \\ 
& \checkmark & \checkmark  &\smallcircle & 84.5 & 91.3 & 87.7 & 87.2 & 71.3 & 93.5 & 80.9 & 77.9 & 63.9 & 95.3 & 76.5 & 70.8 \\ 
& \smallcircle & \checkmark  &\checkmark & 89.6 & 83.2 & 86.3 & 86.8 & 78.2 & 86.1 & 82.0 & \textbf{81.0} & 70.0 & 89.0 & 78.4 & \textbf{75.4} \\ 
& \checkmark & \smallcircle  &\checkmark & 89.6 & 83.2 & 86.3 & 86.8 & 74.5 & 85.3 & 79.5 & 78.0 & 67.3 & 88.8 & 76.6 & 72.9 \\ 
& \checkmark & \checkmark  &\checkmark & 88.4 & 86.0 & 87.2 & 87.3 & 73.1 & 89.7 & 80.6 & 78.4 & 65.1 & 92.6 & 76.5 & 71.5 \\ 
& \multicolumn{3}{c||}{--- SFT LLaVA ---} & 78.8 & 95.0 & 86.2 & 84.7 & 68.4 & 96.5 & 80.0 & 75.9 & 62.4 & 98.1 & 76.3 & 69.5 \\ 
& \multicolumn{3}{c||}{--- Base LLaVA ---} & 64.3 & 93.8 & 76.3 & 68.3 & 58.6 & 94.2 & 72.2 & 62.3 & 57.9 & 96.0 & 72.2 & 61.7 \\ 
\hline 
 \multirow{9}{*}{\centering \textbf{ko}} 
 & \checkmark & \smallcircle  &\smallcircle & 86.8 & 55.4 & 67.7 & 73.3 & 81.1 & 56.7 & 66.7 & 71.5 & 82.0 & 56.2 & 66.7 & 71.5 \\ 
& \smallcircle & \checkmark  &\smallcircle & 90.2 & 51.8 & 65.9 & 70.5 & 86.0 & 52.0 & 64.8 & 68.6 & 87.6 & 48.4 & 62.4 & 67.5 \\ 
& \smallcircle & \smallcircle  &\checkmark & 67.6 & 76.6 & 71.8 & 62.5 & 70.3 & 76.2 & 73.2 & 57.3 & 70.8 & 77.0 & 73.8 & 59.0 \\ 
& \checkmark & \checkmark  &\smallcircle & 86.4 & 67.4 & 75.7 & \textbf{77.9} & 79.5 & 68.3 & 73.5 & \textbf{74.4} & 77.9 & 67.0 & 72.0 & \textbf{73.4} \\ 
& \smallcircle & \checkmark  &\checkmark & 82.2 & 54.7 & 65.7 & 62.0 & 80.6 & 53.8 & 64.5 & 57.4 & 76.8 & 53.3 & 62.9 & 57.2 \\ 
& \checkmark & \smallcircle  &\checkmark & 85.7 & 61.9 & 71.9 & 74.6 & 79.7 & 64.0 & 71.0 & 71.7 & 77.3 & 62.8 & 69.3 & 70.1 \\ 
& \checkmark & \checkmark  &\checkmark & 80.6 & 67.5 & 73.4 & 72.0 & 76.7 & 68.2 & 72.2 & 67.4 & 75.0 & 68.0 & 71.3 & 66.0 \\ 
& \multicolumn{3}{c||}{--- SFT LLaVA ---} & 83.1 & 70.4 & 76.2 & 77.5 & 76.2 & 69.6 & 72.7 & 72.8 & 75.6 & 69.3 & 72.3 & 72.3 \\ 
& \multicolumn{3}{c||}{--- Base LLaVA ---} & 65.2 & 62.0 & 63.5 & 44.7 & 49.8 & 59.8 & 54.4 & 37.2 & 54.5 & 60.4 & 57.3 & 37.5 \\ 
\hline 
 \multirow{9}{*}{\centering \textbf{Avg.}} 
 & \rowcolor{gray!20} \checkmark & \smallcircle  &\smallcircle & 72.8 & 80.4 & 72.3 & 68.4 & 67.6 & 82.2 & 70.8 & 65.7 & 65.1 & 81.6 & 68.9 & 63.4 \\ 
& \rowcolor{gray!20} \smallcircle & \checkmark  &\smallcircle & 72.8 & 70.0 & 63.1 & 58.5 & 68.6 & 72.0 & 62.5 & 56.6 & 67.3 & 70.9 & 60.8 & 54.6 \\ 
& \rowcolor{gray!20} \smallcircle & \smallcircle  &\checkmark & 67.8 & 85.3 & 73.4 & 66.1 & 64.8 & 86.7 & 72.5 & 63.2 & 62.5 & 86.8 & 71.2 & 61.4 \\ 
& \rowcolor{gray!20} \checkmark & \checkmark  &\smallcircle & 73.9 & 79.0 & 71.3 & 68.4 & 68.6 & 80.5 & 69.6 & 65.5 & 65.9 & 79.9 & 67.5 & 62.9 \\ 
& \rowcolor{gray!20} \smallcircle & \checkmark  &\checkmark & 74.1 & 76.9 & 71.8 & 63.2 & 69.9 & 78.2 & 70.5 & 59.6 & 66.0 & 78.6 & 68.4 & 56.8 \\ 
& \rowcolor{gray!20} \checkmark & \smallcircle  &\checkmark & 73.9 & 80.0 & 73.3 & 69.4 & 68.2 & 82.1 & 71.9 & \textbf{66.7} & 65.1 & 81.6 & 69.7 & \textbf{64.0} \\ 
& \rowcolor{gray!20} \checkmark & \checkmark  &\checkmark & 74.4 & 79.0 & 73.4 & \textbf{69.7} & 68.7 & 81.4 & 71.8 & 66.1 & 65.6 & 81.5 & 69.8 & 62.9 \\ 
& \multicolumn{3}{c||}{\cellcolor{gray!20}--- SFT LLaVA ---}  & \rowcolor{gray!20} 70.6 & 82.2 & 71.5 & 66.8 & 66.0 & 83.0 & 69.8 & 64.1 & 64.2 & 82.2 & 68.0 & 62.0 \\ 
& \multicolumn{3}{c||}{\cellcolor{gray!20}--- Base LLaVA ---} & \rowcolor{gray!20} 44.2 & 71.2 & 53.0 & 45.7 & 41.5 & 70.8 & 51.8 & 43.2 & 42.8 & 71.3 & 52.8 & 43.1 \\ 
\hline 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%  END OF AUTO GENENRATE AREA %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\label{tab:full_results_on_ablation_study_ratio}
\end{longtable}


==> tables/high_low_1_2.tex <==
%%%%%%%%%%%%%%%%%%%% MAIN  RESULT POPE TABLE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table*}
\centering
\caption{

We present a comparative analysis of performance across different data ratios, guided by the language resources provided by all three datasets in the POPE benchmark. 
The ratio `x:y' displayed in this table denotes the sample rate for high-resource languages versus that of low-resource languages, while ``Base'' denotes the performance of the base LLaVA 1.5 model. 
Our evaluation is conducted on the ``popular'' dataset subset. Average scores are indicated in a \colorbox{gray!20}{gray} shade while the top accuracy results are highlighted in bold.
}

\begin{tabular}{cc ||ccc|c || ccc|c || ccc|c}

\hline
\multicolumn{2}{c||}{} & \multicolumn{4}{c||}{MS COCO} & \multicolumn{4}{c||}{AOKVQA} & \multicolumn{4}{c}{GQA}\\
\textbf{lang.}& {method.} &Precision & Recall & F1 & Accuracy & Precision & Recall & F1 & Accuracy & Precision & Recall & F1 & Accuracy\\
\hline
\hline


\multicolumn{14}{c}{\textbf{High Resource Languages (HRL)}} \\   \hline 
 \multirow{3}{*}{\centering \textbf{en}} 
 & Base & 94.6 & 78.1 & 85.6 & \textbf{86.0} & 87.9 & 87.0 & 87.4 & \textbf{86.8} & 83.0 & 84.0 & 83.5 & 82.8 \\ 
& 1:1 & 97.2 & 72.1 & 82.8 & 85.0 & 91.8 & 78.9 & 84.9 & 85.9 & 87.7 & 76.8 & 81.9 & 83.0 \\ 
& 1:2 & 97.1 & 72.0 & 82.7 & 84.9 & 91.4 & 79.5 & 85.1 & 86.0 & 86.7 & 78.0 & 82.1 & \textbf{83.0} \\ 
\hline 
 \multirow{3}{*}{\centering \textbf{ru}} 
 & Base & 53.6 & 98.4 & 69.4 & 55.9 & 52.1 & 99.9 & 68.5 & 53.9 & 52.6 & 99.7 & 68.9 & 54.8 \\ 
& 1:1 & 77.7 & 93.0 & 84.7 & \textbf{83.1} & 63.3 & 97.9 & 76.9 & \textbf{70.6} & 58.0 & 98.1 & 72.9 & \textbf{63.5} \\ 
& 1:2 & 73.3 & 94.8 & 82.7 & 80.1 & 60.9 & 98.9 & 75.4 & 67.7 & 56.6 & 98.8 & 72.0 & 61.5 \\ 
\hline 
 \multirow{3}{*}{\centering \textbf{de}} 
 & Base & 95.2 & 75.0 & 83.9 & 83.3 & 88.6 & 73.3 & 80.2 & 80.4 & 80.4 & 72.8 & 76.4 & 75.8 \\ 
& 1:1 & 95.9 & 71.9 & 82.2 & 84.4 & 89.5 & 73.1 & 80.4 & 82.2 & 80.7 & 72.0 & 76.1 & 77.4 \\ 
& 1:2 & 95.7 & 74.3 & 83.7 & \textbf{85.5} & 88.1 & 76.1 & 81.7 & \textbf{82.9} & 79.4 & 74.7 & 77.0 & \textbf{77.7} \\ 
\hline 
 \multirow{3}{*}{\centering \textbf{zh}} 
 & Base & 50.0 & 100.0 & 66.6 & 47.8 & 49.9 & 100.0 & 66.6 & 48.1 & 49.5 & 100.0 & 66.2 & 47.6 \\ 
& 1:1 & 81.3 & 92.9 & 86.7 & \textbf{85.8} & 67.7 & 97.4 & 79.9 & \textbf{75.5} & 62.8 & 96.9 & 76.2 & \textbf{69.7} \\ 
& 1:2 & 76.0 & 95.0 & 84.4 & 82.5 & 63.3 & 98.3 & 77.0 & 70.7 & 60.1 & 98.6 & 74.7 & 66.5 \\ 
\hline 
 \multirow{3}{*}{\centering \textbf{ja}} 
 & Base & 51.2 & 100.0 & 67.7 & 49.1 & 49.9 & 100.0 & 66.6 & 48.3 & 49.6 & 100.0 & 66.3 & 47.5 \\ 
& 1:1 & 87.8 & 85.8 & 86.8 & \textbf{86.9} & 68.1 & 91.3 & 78.0 & \textbf{74.2} & 62.9 & 91.3 & 74.5 & \textbf{68.7} \\ 
& 1:2 & 83.9 & 89.9 & 86.8 & 86.3 & 64.2 & 94.7 & 76.5 & 70.9 & 59.0 & 95.4 & 72.9 & 64.5 \\ 
\hline 
 \multirow{3}{*}{\centering \textbf{fr}} 
 & Base & 63.7 & 97.9 & 77.2 & 70.9 & 62.4 & 99.4 & 76.7 & 69.6 & 58.5 & 99.5 & 73.7 & 64.3 \\ 
& 1:1 & 81.7 & 92.7 & 86.9 & \textbf{86.0} & 69.3 & 96.8 & 80.8 & \textbf{77.0} & 63.2 & 98.3 & 76.9 & \textbf{70.5} \\ 
& 1:2 & 79.6 & 93.7 & 86.1 & 84.8 & 67.3 & 98.0 & 79.8 & 75.2 & 61.6 & 98.7 & 75.9 & 68.6 \\ 
\hline 
 \multirow{3}{*}{\centering \textbf{es}} 
 & Base & 97.7 & 47.7 & 64.1 & 73.2 & 95.9 & 48.3 & 64.2 & 73.0 & 95.8 & 47.3 & 63.3 & 72.6 \\ 
& 1:1 & 94.3 & 77.3 & 85.0 & 86.3 & 84.0 & 83.5 & 83.8 & \textbf{83.8} & 77.6 & 81.5 & 79.5 & \textbf{78.9} \\ 
& 1:2 & 93.3 & 79.7 & 86.0 & \textbf{86.9} & 81.8 & 86.6 & 84.1 & 83.7 & 74.9 & 86.1 & 80.1 & 78.6 \\ 
\hline 
 \multirow{3}{*}{\centering \textbf{pt}} 
 & Base & 64.4 & 97.8 & 77.7 & 70.8 & 60.5 & 99.5 & 75.2 & 66.6 & 57.5 & 99.7 & 73.0 & 62.6 \\ 
& 1:1 & 80.3 & 91.7 & 85.6 & \textbf{84.6} & 68.1 & 96.5 & 79.8 & \textbf{75.6} & 62.0 & 97.0 & 75.7 & \textbf{68.8} \\ 
& 1:2 & 77.5 & 93.2 & 84.6 & 83.0 & 66.4 & 97.5 & 79.0 & 74.1 & 60.9 & 98.1 & 75.2 & 67.6 \\ 
\hline 
 \multirow{3}{*}{\centering \textbf{Avg.}} 
 & \rowcolor{gray!20} Base & 71.3 & 86.9 & 74.0 & 67.1 & 68.4 & 88.4 & 73.2 & 65.8 & 65.9 & 87.9 & 71.4 & 63.5 \\ 
& \rowcolor{gray!20} 1:1 & 87.0 & 84.7 & 85.1 & \textbf{85.3} & 75.2 & 89.4 & 80.6 & \textbf{78.1} & 69.4 & 89.0 & 76.7 & \textbf{72.6} \\ 
& \rowcolor{gray!20} 1:2 & 84.5 & 86.6 & 84.6 & 84.3 & 72.9 & 91.2 & 79.8 & 76.4 & 67.4 & 91.1 & 76.2 & 71.0 \\ 
\hline 
\multicolumn{14}{c}{\textbf{Low Resource Languages (LRL)}} \\  \hline 
 \multirow{3}{*}{\centering \textbf{uk}} 
 & Base & 41.6 & 100.0 & 58.8 & 16.8 & 49.7 & 100.0 & 66.4 & 18.2 & 52.3 & 100.0 & 68.7 & 18.3 \\ 
& 1:1 & 49.6 & 99.1 & 66.1 & \textbf{48.4} & 49.2 & 99.3 & 65.8 & \textbf{48.1} & 49.4 & 99.1 & 65.9 & \textbf{47.8} \\ 
& 1:2 & 49.5 & 98.8 & 66.0 & 48.0 & 49.1 & 99.2 & 65.7 & 47.6 & 49.1 & 99.0 & 65.6 & 47.1 \\ 
\hline 
 \multirow{3}{*}{\centering \textbf{bg}} 
 & Base & 49.8 & 100.0 & 66.5 & 48.7 & 49.3 & 100.0 & 66.0 & 48.5 & 49.3 & 100.0 & 66.0 & 48.5 \\ 
& 1:1 & 58.2 & 95.8 & 72.4 & \textbf{63.5} & 57.6 & 98.9 & 72.8 & \textbf{63.0} & 55.2 & 98.9 & 70.8 & \textbf{59.3} \\ 
& 1:2 & 56.5 & 97.1 & 71.4 & 61.1 & 55.7 & 99.4 & 71.4 & 60.2 & 54.0 & 99.2 & 69.9 & 57.3 \\ 
\hline 
 \multirow{3}{*}{\centering \textbf{tr}} 
 & Base & 0.0 & 0.0 & 0.0 & 49.7 & 0.0 & 0.0 & 0.0 & 49.9 & 0.0 & 0.0 & 0.0 & 49.7 \\ 
& 1:1 & 91.3 & 51.6 & 65.9 & \textbf{73.2} & 84.7 & 55.0 & 66.7 & \textbf{72.4} & 79.2 & 51.2 & 62.2 & \textbf{68.8} \\ 
& 1:2 & 91.4 & 49.0 & 63.8 & 72.1 & 83.2 & 53.0 & 64.8 & 71.1 & 79.1 & 49.6 & 61.0 & 68.1 \\ 
\hline 
 \multirow{3}{*}{\centering \textbf{ar}} 
 & Base & 64.3 & 93.8 & 76.3 & 68.3 & 58.6 & 94.2 & 72.2 & 62.3 & 57.9 & 96.0 & 72.2 & 61.7 \\ 
& 1:1 & 87.5 & 87.8 & 87.7 & 87.6 & 72.8 & 90.9 & 80.9 & \textbf{78.5} & 65.1 & 92.3 & 76.4 & \textbf{71.5} \\ 
& 1:2 & 86.1 & 91.0 & 88.5 & \textbf{88.1} & 71.3 & 93.1 & 80.8 & 77.8 & 64.2 & 95.7 & 76.8 & 71.2 \\ 
\hline 
 \multirow{3}{*}{\centering \textbf{ko}} 
 & Base & 65.2 & 62.0 & 63.5 & 44.7 & 49.8 & 59.8 & 54.4 & 37.2 & 54.5 & 60.4 & 57.3 & 37.5 \\ 
& 1:1 & 89.4 & 60.2 & 72.0 & \textbf{75.5} & 82.2 & 61.7 & 70.5 & \textbf{72.4} & 80.0 & 60.1 & 68.6 & \textbf{71.0} \\ 
& 1:2 & 87.3 & 60.6 & 71.6 & 74.5 & 80.5 & 62.9 & 70.6 & 70.7 & 78.7 & 61.0 & 68.8 & 69.3 \\ 
\hline 
 \multirow{3}{*}{\centering \textbf{Avg.}} 
 & \rowcolor{gray!20} Base & 44.2 & 71.2 & 53.0 & 45.7 & 41.5 & 70.8 & 51.8 & 43.2 & 42.8 & 71.3 & 52.8 & 43.1 \\ 
& \rowcolor{gray!20} 1:1 & 75.2 & 78.9 & 72.8 & \textbf{69.7} & 69.3 & 81.2 & 71.3 & \textbf{66.9} & 65.8 & 80.3 & 68.8 & \textbf{63.7} \\ 
& \rowcolor{gray!20} 1:2 & 74.2 & 79.3 & 72.2 & 68.8 & 68.0 & 81.5 & 70.6 & 65.5 & 65.0 & 80.9 & 68.4 & 62.6 \\ 
\hline 




\hline\hline

\end{tabular}
% }
\label{tab:high_low_1_2}
\end{table*}


==> tables/pope_adversarial.tex <==


\begin{table*}
\centering
\caption{

A comparative evaluation of performance metrics between base LLaVA-1.5 and our model on the remaining two styles of all three datasets in the POPE MUL benchmark. 
Details concerning the `popular' style can be found in the main body of the paper. The average scores are marked in \colorbox{gray!20}{gray} and bold text denotes the best accuracy results.
}

\resizebox{15.8cm}{!}{
\begin{tabular}{c|cc ||ccc|c || ccc|c || ccc|c}

\hline
&\multicolumn{2}{c||}{} & \multicolumn{4}{c||}{MS COCO} & \multicolumn{4}{c||}{AOKVQA} & \multicolumn{4}{c}{GQA}\\
\textbf{Style.}&\textbf{lang.}& {method.} &Precision & Recall & F1 & Accuracy & Precision & Recall & F1 & Accuracy & Precision & Recall & F1 & Accuracy\\
\hline



 
 \multirow{32}{*}{\centering \textbf{adversarial}} &\multicolumn{14}{c}{\textbf{High Resource Languages (HRL)}} \\   \hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|} 
& \multirow{2}{*}{\centering \textbf{en}} 
 & Base & 90.1 & 78.3 & 83.8 & \textbf{84.8} & 77.6 & 87.0 & 82.0 & \textbf{80.9} & 79.3 & 84.1 & 81.7 & \textbf{81.1} \\ 
&& Ours & 93.6 & 70.7 & 80.5 & 82.9 & 81.7 & 77.3 & 79.4 & 80.0 & 83.6 & 76.1 & 79.7 & 80.6 \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& \multirow{2}{*}{\centering \textbf{ru}} 
 & Base & 53.6 & 98.5 & 69.4 & 56.5 & 52.7 & 99.9 & 69.0 & 55.0 & 53.0 & 99.7 & 69.2 & 55.7 \\ 
&& Ours & 72.2 & 91.4 & 80.7 & \textbf{76.9} & 60.4 & 96.4 & 74.3 & \textbf{66.5} & 59.7 & 97.3 & 73.9 & \textbf{65.5} \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& \multirow{2}{*}{\centering \textbf{de}} 
 & Base & 89.3 & 75.3 & 81.7 & \textbf{83.1} & 81.4 & 73.4 & 77.2 & \textbf{78.3} & 81.5 & 73.5 & 77.3 & \textbf{78.4} \\ 
&& Ours & 91.0 & 70.4 & 79.4 & 81.7 & 81.2 & 70.5 & 75.5 & 77.1 & 82.1 & 71.1 & 76.2 & 77.8 \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& \multirow{2}{*}{\centering \textbf{zh}} 
 & Base & 50.1 & 100.0 & 66.7 & 50.1 & 50.0 & 99.9 & 66.7 & 50.1 & 50.1 & 100.0 & 66.7 & 50.1 \\ 
&& Ours & 71.5 & 91.6 & 80.3 & \textbf{77.5} & 61.0 & 96.5 & 74.8 & \textbf{67.4} & 60.6 & 97.1 & 74.6 & \textbf{67.0} \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& \multirow{2}{*}{\centering \textbf{ja}} 
 & Base & 50.3 & 100.0 & 66.9 & 50.6 & 50.2 & 100.0 & 66.8 & 50.4 & 50.0 & 100.0 & 66.7 & 50.0 \\ 
&& Ours & 76.3 & 87.0 & 81.3 & \textbf{80.0} & 62.2 & 91.5 & 74.0 & \textbf{67.9} & 63.0 & 93.3 & 75.2 & \textbf{69.3} \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& \multirow{2}{*}{\centering \textbf{fr}} 
 & Base & 58.6 & 97.7 & 73.3 & 64.4 & 56.6 & 99.4 & 72.2 & 61.7 & 56.2 & 99.5 & 71.8 & 60.9 \\ 
&& Ours & 74.7 & 91.5 & 82.3 & \textbf{80.3} & 61.5 & 95.8 & 74.9 & \textbf{67.9} & 61.5 & 97.1 & 75.3 & \textbf{68.2} \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& \multirow{2}{*}{\centering \textbf{es}} 
 & Base & 96.6 & 47.3 & 63.5 & 72.8 & 87.6 & 48.1 & 62.1 & 70.6 & 91.5 & 48.2 & 63.1 & 71.9 \\ 
&& Ours & 88.5 & 76.3 & 81.9 & \textbf{82.6} & 73.4 & 83.4 & 78.1 & \textbf{76.5} & 75.2 & 84.1 & 79.4 & \textbf{77.9} \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& \multirow{2}{*}{\centering \textbf{pt}} 
 & Base & 59.0 & 97.7 & 73.6 & 64.9 & 56.0 & 99.5 & 71.7 & 60.7 & 56.2 & 99.7 & 71.9 & 61.0 \\ 
&& Ours & 70.6 & 90.6 & 79.4 & \textbf{76.5} & 60.4 & 95.1 & 73.9 & \textbf{66.4} & 60.0 & 95.9 & 73.8 & \textbf{66.0} \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& \multirow{2}{*}{\centering \textbf{Avg.}} 
 & \rowcolor{gray!20} Base & 68.4 & 86.9 & 72.4 & 65.9 & 64.0 & 88.4 & 70.9 & 63.5 & 64.7 & 88.1 & 71.0 & 63.6 \\ 
&& \rowcolor{gray!20} Ours & 79.8 & 83.7 & 80.7 & \textbf{79.8} & 67.7 & 88.3 & 75.6 & \textbf{71.2} & 68.2 & 89.0 & 76.0 & \textbf{71.5} \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
&\multicolumn{14}{c}{\textbf{Low Resource Languages (LRL)}} \\  \hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|} 
& \multirow{2}{*}{\centering \textbf{uk}} 
 & Base & 49.2 & 100.0 & 65.9 & 17.1 & 47.5 & 100.0 & 64.4 & 18.6 & 47.3 & 100.0 & 64.2 & 18.9 \\ 
&& Ours & 50.9 & 98.6 & 67.1 & \textbf{49.4} & 50.1 & 99.6 & 66.7 & \textbf{48.3} & 49.8 & 99.5 & 66.4 & \textbf{48.3} \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& \multirow{2}{*}{\centering \textbf{bg}} 
 & Base & 50.1 & 100.0 & 66.7 & 50.1 & 50.1 & 100.0 & 66.7 & 50.1 & 50.0 & 100.0 & 66.7 & 50.0 \\ 
&& Ours & 61.8 & 92.5 & 74.1 & \textbf{67.0} & 56.9 & 95.1 & 71.2 & \textbf{60.0} & 57.1 & 97.4 & 72.0 & \textbf{60.4} \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& \multirow{2}{*}{\centering \textbf{tr}} 
 & Base & 0.0 & 0.0 & 0.0 & 50.0 & 0.0 & 0.0 & 0.0 & 50.0 & 0.0 & 0.0 & 0.0 & 50.0 \\ 
&& Ours & 79.5 & 50.4 & 61.7 & \textbf{67.9} & 69.9 & 52.6 & 60.1 & \textbf{64.1} & 71.9 & 49.5 & 58.6 & \textbf{64.0} \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& \multirow{2}{*}{\centering \textbf{ar}} 
 & Base & 61.2 & 93.8 & 74.1 & 67.1 & 57.0 & 94.7 & 71.1 & 61.6 & 57.6 & 96.3 & 72.1 & 62.7 \\ 
&& Ours & 72.3 & 85.8 & 78.5 & \textbf{76.5} & 64.8 & 89.3 & 75.1 & \textbf{70.4} & 64.4 & 93.0 & 76.1 & \textbf{70.8} \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& \multirow{2}{*}{\centering \textbf{ko}} 
 & Base & 58.6 & 62.7 & 60.6 & 41.7 & 48.2 & 64.0 & 55.0 & 33.7 & 52.5 & 63.0 & 57.2 & 36.2 \\ 
&& Ours & 74.6 & 66.5 & 70.4 & \textbf{67.6} & 70.1 & 68.1 & 69.1 & \textbf{63.7} & 70.6 & 68.7 & 69.6 & \textbf{63.7} \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& \multirow{2}{*}{\centering \textbf{Avg.}} 
 & \rowcolor{gray!20} Base & 43.8 & 71.3 & 53.5 & 45.2 & 40.5 & 71.8 & 51.4 & 42.8 & 41.5 & 71.8 & 52.0 & 43.5 \\ 
&& \rowcolor{gray!20} Ours & 67.8 & 78.8 & 70.4 & \textbf{65.7} & 62.4 & 81.0 & 68.4 & \textbf{61.3} & 62.8 & 81.6 & 68.5 & \textbf{61.4} \\ 
 \hline 
 \multirow{32}{*}{\centering \textbf{random}} &\multicolumn{14}{c}{\textbf{High Resource Languages (HRL)}} \\   \hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|} 
& \multirow{2}{*}{\centering \textbf{en}} 
 & Base & 97.0 & 78.3 & 86.7 & \textbf{88.0} & 93.6 & 87.0 & 90.2 & \textbf{90.5} & 92.0 & 84.1 & 87.9 & \textbf{88.4} \\ 
&& Ours & 98.8 & 70.7 & 82.4 & 84.9 & 96.0 & 77.3 & 85.6 & 87.0 & 95.5 & 76.1 & 84.7 & 86.2 \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& \multirow{2}{*}{\centering \textbf{ru}} 
 & Base & 53.2 & 98.3 & 69.0 & 55.8 & 53.2 & 99.9 & 69.4 & 56.0 & 53.1 & 99.7 & 69.3 & 55.9 \\ 
&& Ours & 77.3 & 91.7 & 83.9 & \textbf{79.2} & 68.3 & 96.4 & 79.9 & \textbf{73.2} & 67.8 & 97.2 & 79.9 & \textbf{73.3} \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& \multirow{2}{*}{\centering \textbf{de}} 
 & Base & 96.1 & 74.5 & 84.0 & \textbf{85.8} & 93.4 & 73.9 & 82.5 & \textbf{84.3} & 91.8 & 72.4 & 81.0 & \textbf{83.0} \\ 
&& Ours & 96.9 & 69.9 & 81.2 & 83.8 & 92.0 & 70.1 & 79.6 & 82.0 & 92.0 & 71.0 & 80.2 & 82.4 \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& \multirow{2}{*}{\centering \textbf{zh}} 
 & Base & 50.1 & 100.0 & 66.8 & 50.2 & 50.1 & 100.0 & 66.7 & 50.1 & 50.1 & 100.0 & 66.7 & 50.2 \\ 
&& Ours & 75.6 & 91.2 & 82.7 & \textbf{80.8} & 68.1 & 96.7 & 79.9 & \textbf{75.7} & 69.2 & 96.9 & 80.7 & \textbf{76.9} \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& \multirow{2}{*}{\centering \textbf{ja}} 
 & Base & 50.2 & 99.9 & 66.9 & 50.5 & 50.2 & 100.0 & 66.9 & 50.5 & 50.1 & 100.0 & 66.7 & 50.2 \\ 
&& Ours & 83.6 & 87.1 & 85.3 & \textbf{84.9} & 75.5 & 91.7 & 82.8 & \textbf{80.9} & 75.0 & 93.3 & 83.2 & \textbf{81.1} \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& \multirow{2}{*}{\centering \textbf{fr}} 
 & Base & 59.0 & 97.5 & 73.5 & 64.9 & 57.1 & 99.4 & 72.5 & 62.3 & 57.4 & 99.5 & 72.8 & 62.8 \\ 
&& Ours & 78.6 & 91.3 & 84.5 & \textbf{83.2} & 69.9 & 95.7 & 80.8 & \textbf{77.2} & 70.8 & 97.2 & 81.9 & \textbf{78.6} \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& \multirow{2}{*}{\centering \textbf{es}} 
 & Base & 98.9 & 47.5 & 64.2 & 73.5 & 96.5 & 47.9 & 64.0 & 73.1 & 95.5 & 48.0 & 63.9 & 72.9 \\ 
&& Ours & 92.4 & 76.5 & 83.7 & \textbf{84.6} & 87.7 & 83.2 & 85.4 & \textbf{85.6} & 85.2 & 84.0 & 84.6 & \textbf{84.4} \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& \multirow{2}{*}{\centering \textbf{pt}} 
 & Base & 58.3 & 97.7 & 73.0 & 63.8 & 55.6 & 99.5 & 71.3 & 60.0 & 56.4 & 99.8 & 72.1 & 61.3 \\ 
&& Ours & 71.1 & 90.7 & 79.7 & \textbf{76.9} & 64.0 & 95.5 & 76.7 & \textbf{70.9} & 65.1 & 96.3 & 77.7 & \textbf{72.3} \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& \multirow{2}{*}{\centering \textbf{Avg.}} 
 & \rowcolor{gray!20} Base & 70.3 & 86.7 & 73.0 & 66.6 & 68.7 & 88.4 & 72.9 & 65.9 & 68.3 & 88.0 & 72.5 & 65.6 \\ 
&& \rowcolor{gray!20} Ours & 84.3 & 83.6 & 82.9 & \textbf{82.3} & 77.7 & 88.3 & 81.3 & \textbf{79.1} & 77.6 & 89.0 & 81.6 & \textbf{79.4} \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
&\multicolumn{14}{c}{\textbf{Low Resource Languages (LRL)}} \\  \hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|} 
& \multirow{2}{*}{\centering \textbf{uk}} 
 & Base & 51.3 & 100.0 & 67.8 & 17.0 & 50.0 & 100.0 & 66.7 & 18.5 & 49.1 & 100.0 & 65.8 & 18.8 \\ 
&& Ours & 50.5 & 98.6 & 66.8 & \textbf{49.0} & 49.9 & 99.4 & 66.4 & \textbf{48.4} & 50.3 & 99.4 & 66.8 & \textbf{48.9} \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& \multirow{2}{*}{\centering \textbf{bg}} 
 & Base & 50.1 & 100.0 & 66.7 & 50.2 & 50.0 & 100.0 & 66.7 & 50.0 & 50.0 & 100.0 & 66.7 & 50.0 \\ 
&& Ours & 61.1 & 92.4 & 73.6 & \textbf{66.4} & 57.8 & 95.5 & 72.0 & \textbf{62.1} & 57.8 & 97.7 & 72.6 & \textbf{62.6} \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& \multirow{2}{*}{\centering \textbf{tr}} 
 & Base & 0.0 & 0.0 & 0.0 & 50.0 & 0.0 & 0.0 & 0.0 & 50.0 & 0.0 & 0.0 & 0.0 & 50.0 \\ 
&& Ours & 78.4 & 48.8 & 60.2 & \textbf{66.8} & 77.8 & 54.3 & 64.0 & \textbf{68.1} & 76.6 & 50.7 & 61.0 & \textbf{66.4} \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& \multirow{2}{*}{\centering \textbf{ar}} 
 & Base & 53.2 & 93.7 & 67.9 & 55.7 & 53.4 & 94.9 & 68.3 & 56.0 & 54.0 & 96.4 & 69.2 & 57.1 \\ 
&& Ours & 63.7 & 85.8 & 73.1 & \textbf{68.5} & 61.2 & 89.4 & 72.7 & \textbf{66.4} & 63.5 & 92.9 & 75.4 & \textbf{69.7} \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& \multirow{2}{*}{\centering \textbf{ko}} 
 & Base & 58.7 & 62.5 & 60.6 & 47.7 & 47.8 & 63.2 & 54.4 & 41.9 & 52.6 & 62.6 & 57.2 & 43.7 \\ 
&& Ours & 80.9 & 67.5 & 73.6 & \textbf{71.0} & 76.5 & 68.1 & 72.1 & \textbf{67.6} & 77.6 & 68.0 & 72.5 & \textbf{68.3} \\ 
\hhline{|~|-|-|-|-|-|-|-|-|-|-|-|-|-|-|}
& \multirow{2}{*}{\centering \textbf{Avg.}} 
 & \rowcolor{gray!20} Base & 42.7 & 71.2 & 52.6 & 44.1 & 40.2 & 71.6 & 51.2 & 43.3 & 41.1 & 71.8 & 51.8 & 43.9 \\ 
&& \rowcolor{gray!20} Ours & 66.9 & 78.6 & 69.5 & \textbf{64.3} & 64.6 & 81.4 & 69.4 & \textbf{62.5} & 65.1 & 81.7 & 69.7 & \textbf{63.2} \\ 
 \hline 



\hline\hline

\end{tabular}}
\label{tab:pope_adversarial}
\end{table*}

